Deep Weakly Supervised Positioning

PoseNet can map a photo to the position where it is taken, which is appealing in robotics. However, training PoseNet requires full supervision, where ground truth positions are non-trivial to obtain. Can we train PoseNet without knowing the ground truth positions for each observation? We show that this is possible via constraint-based weak-supervision, leading to the proposed framework: DeepGPS. Particularly, using wheel-encoder-estimated distances traveled by a robot along random straight line segments as constraints between PoseNet outputs, DeepGPS can achieve a relative positioning error of less than 2%. Moreover, training DeepGPS can be done as auto-calibration with almost no human attendance, which is more attractive than its competing methods that typically require careful and expert-level manual calibration. We conduct various experiments on simulated and real datasets to demonstrate the general applicability, effectiveness, and accuracy of DeepGPS, and perform a comprehensive analysis of its robustness. Our code is available at https://ai4ce.github.io/DeepGPS/.

==> 2-related_works.tex <==
\section{Related Works}
\label{sec:related_works}
\begin{table*}[!t]
\centering
\caption{A brief qualitative summary of common positioning technologies (row 2--6)~\cite{brena2017evolution,zafari2019survey} and algorithms (row 7--11). Easy-setup means calibration/train\-ing/mapping is automatic or not required. Applicability means whether an algorithm suits for different sensing modalities. I/O means indoor/outdoor scenes. ``\texttildelow'' means the accuracy is high around training trajectories but low elsewhere. \nr{Several comments from reviewers on this tables: (1) ``Accuracy-level'' seems slightly arbitrary; (2) Why is VSLAM not map-free? You don't need a prior map unless the system is localizing against a pre-built SLAM map, in which case it's no longer doing any mapping.); (3) ``Particle filter'' is an estimation framework rather than localization method;} \label{table:compare}}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|cccccc}
\toprule
Method & Typical-scene \qquad & Applicability \qquad & Map-free \qquad & Infrastructure-free \qquad & Easy-setup \qquad & Accuracy-level \\\midrule
Vicon\textsuperscript{\textregistered} & I & N/A & $\checkmark$ & & & +++\\
Ultrasound & I & N/A & $\checkmark$ & & & ++\\
WiFi      & I & N/A & $\checkmark$ & & & -\\
UWB       & I & N/A & $\checkmark$ & & & ++ \\
GPS             & O & N/A & $\checkmark$ & & $\checkmark$ & +\\ \midrule
VSLAM & I\&O & & & $\checkmark$ &  & ++\\
Particle Filter & I\&O & $\checkmark$ & & $\checkmark$ &  & ++\\
PoseNet         & I\&O & $\checkmark$ & $\checkmark$ & $\checkmark$ & & \texttildelow\\
DeepMapping     & I\&O & & & $\checkmark$ & $\checkmark$ & \texttildelow\\
\textbf{DeepGPS}         & I\&O & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & ++\\
\bottomrule
\end{tabular}%
% \vspace{-3mm}
}
\end{table*}
%\chen{we need 2 pages for related works.}
%We review the prior works on place recognition/localization and visual odometry, and provide a brief summary on ... (learning methods that do not require fully labeled dataset... TBDTBDTBD)

%\textbf{Positioning system:} % briefly introduce PS, then focus on vision-based PS

There has been a large body of work on indoor/outdoor positioning using various sensing modalities. We provide a brief qualitative summary in Table~\ref{table:compare} and refer our readers to~\cite{brena2017evolution,zafari2019survey} for comprehensive surveys of non-vision-based methods. Next, we focus our discussion on vision-based methods.

%\begin{flushleft}
\noindent\textbf{Visual localization.} Prior works on visual localization generally fall into two groups. The methods in the first category are based on matching features between the local and the global scene. The scene environment can be explicitly represented as a 3D model, which is reconstructed from images or directly captured by 3D scanners. The correspondences can be established by matching hand-crafted~\cite{Lowe:SIFT:IJCV04,Rublee:ORB:ICCV11,Rusu:FPFH:ICRA09,Tombari:SHOT:ECCV10} or learning-based~\cite{Deng:PPFNet:CVPR18,Yew:3DFeatNet:ECCV18,Moo:Learn2FindCrspd:CVPR18,Zeng:3DMatch:CVPR18,Gojcic:PerfectMatch:CVPR19,Dube:SegMatch:ICRA17,Dube:SegMap:RSS18} feature descriptors. Furthermore, image retrieval techniques can also be performed to find the image-level correspondence~\cite{Ding:CamNet:ICCV19,Taira:GeoSemanPoseVerfVisualLoc:ICCV19,Camposeco:HybdCamLoc:CVPR18}. The downside is that these approaches require an explicit representation of the 3D model or have to store all descriptors and camera poses in memory. Additionally, several works use machine learning and deep learning methods to directly regress 3D coordinates of pixels in the image~\cite{Brachmann:DSAC:CVPR17,Sattler:ActSearch:PAMI17,Brachmann:LearnLessMore6DCamLoc:CVPR18,Shotton:SceneCoordReg:CVPR13,Cavallari:RegForestCamLoc:CVPR17,Massiceti:RFvsNNCamLoc:ICRA17,Cavallari:AdapSceneCoordReg:3DV19,Guzman:MultiOutputCamLoc:CVPR14,Cai:CamLocMVConstraint:ICCVW19}. While learning to predict 3D coordinates from image patches yields accurate sensor poses, these approaches may fail to handle large-scale scene~\cite{Taira:InLoc:CVPR18,Schonberger:SemanticVisLoc:CVPR18}.
% \chen{@Li, should we talk a bit about the Particle-Filter based localization?} \nr{TBD}

Rather than learning to find corresponding points between local and global scene, another type of learning-based approach, absolute pose regression (APR), use DNNs to model the full localization pipeline. In this scenario, the global environment is implicitly represented by the weights of DNNs. The core idea is to build DNN models to directly predict the sensor positions for the input observations. The first APR-based approach is PoseNet~\cite{Kendall:PoseNet:ICCV2015} that uses a modified GoogLeNet~\cite{SzegedyGoogLeNet:CVPR15} to regress camera poses. The network is trained by minimizing the Euclidean distance between the predicted poses and the ground truth poses. Since then, the APR-based approach for visual localization has been explored extensively. For example, methods in~\cite{Kendall:GeoLoss4PoseReg:CVPR2017,Kendall:MdlUncertCamLoc:ICRA16} incorporate additional loss terms such as the reprojection error and the weighted position and rotation loss. In addition to the novel loss function, different network architectures are proposed for extracting the fine-grained features~\cite{Melekhov:CamLocHourglassNet:ICCVW17} or for handling sequences of inputs~\cite{Walch:CamLocLSTMStrctFeatCorr:ICCV17,Henriques:MapNetRNN:CVPR18}. Moreover, view synthesis techniques~\cite{Wu:DelveCNN4CamLoc:ICRA2017,Purkait:SynView4APR:BMVC2018,Naseer:RegMonoCam6DOFOutdoor:IROS2017} are integrated into the APR-based approach to enlarge the training dataset and to pose constraints on sensor poses. Methods in~\cite{Brahmbhatt:GeoLearnMap4CamLoc:CVPR18,Radwan:VLocNetPP:RAL18,Valada:VLocNet:ICRA18,Balntas:RelocNet:ECCV18} exploit other available supervision signals, including GPS, IMU, and VO, to improve the accuracy of localization. Despite various network architectures and loss functions, these methods follow the supervised pipeline and require a fully labeled training dataset that contains a massive amount of local observations and the associated ground truth positions. As noted in Section~\ref{sec:intro}, such ground truth positions are not trivial to obtain and therefore pose a big challenge for this supervised learning approach to be effectively deployed in real-world applications.

%\begin{flushleft}
\noindent\textbf{Learning-based visual odometry.} Another related problem to visual localization is the visual odometry (VO) that incrementally estimates the ego-motion of the sensor using a sequence of observations. In our discussion, we briefly review the learning-based VO and refer readers to the survey papers~\cite{Scaramuzza:VOSurveyPart1:RAM11,Fraundorfer:VOSurveyPart2:RAM12} for broader context on the conventional methods. DeepVO~\cite{Wang:DeepVO:ICRA2017} and VidLOc~\cite{Clark:VidLoc:CVPR2017} propose to use a combined CNN and LSTM networks for monocular VO by taking the advantage that CNN and LSTM are capable to extract features from the input images and to incorporate temporal information, respectively. In addition to monocular camera, different sensors are incorporated into learning-based method that allow the information from independent sensors to be fused in a complementary way, including lidar~\cite{Ma:SelSupLidar&cam:ICRA2019}, GPS~\cite{Pillai:TowVEGO;IROS2017}, or IMU~\cite{Clark:VINet:AAAI2017,Wang:LearnInertia:ICASSP2019}. Several works focus on unsupervised learning for the VO problem by jointly estimating the depth maps for the input RGB images~\cite{Mahjourian:UnsupDepthEgoMonGeoConst:CVPR18,Zhou:SfMLearner:CVPR17,Li:UnDeepVO:ICRA2018}. 


%Recently, UnDeepVO [40] present a network constituted by depth and pose estimator which  training  with  consecutive  stereo  images  and  testing  on monocular images. Other depth based methods, [73, 3, 81], also solved through a combination network of depth generation and pose regression. The benefit of involving depth information is that these approaches could recover the absolute scale during estimating the pose.
% Recurrent neural network (RNN) is widely used network architecture for VO task that deals with sequential input. 

%The development of learning-based VO mainly relies on sensor fusion, sequential images and depth information. Fusing independent sensors allow the information to be used in a complementary way~\cite{Pillai:TowVEGO;IROS2017}. For visual-inertial odometry (VIO), VINet~\cite{Clark:VINet:AAAI2017} takes the monocular RGB images and the 6-dimension Inertial Measurement Unit (IMU) data as input to predict the camera motions. Method in~\cite{Shamwell:UnsupVIOwizOLErr:TPAMI2019} introduces the VIO Learner to online correct feed-forward error and avoid trajectory divergences by generating hypothesis trajectories. Method in~\cite{Wang:LearnInertia:ICASSP2019} designs a novel inertia loss and dynamic hard-edge mask to predict camera motions under high speed motion.%All the above learning based methods are dependent on IMU.

% Recurrent convolutional neural network (RCNN) is widely used for training sequential images to study ego-motion of camera. VidLoc~\cite{Clark:VidLoc:CVPR2017} explored bidirectional long short-term memory (LSTM) from sequential images to predict global position and obtaining the instantaneous covariances for pose estimation.
%

%
% Depth based unsupervised sfmlearne~\citehere{}
% Recently, UnDeepVO [40] present a network constituted by depth and pose estimator which  training  with  consecutive  stereo  images  and  testing  on monocular images. Other depth based methods, [73, 3, 81], also solved through a combination network of depth generation and pose regression. The benefit of involving depth information is that these approaches could recover the absolute scale during estimating the pose.
%In our method, we only required monocular RGB images instead of depth information to complete pose and localization estimation.


% \begin{itemize}    
%     \item  DeepVO~\cite{Wang:DeepVO:ICRA2017} demonstrated their CNN-LTSM network by using sequential RGB images without additional sensor data.
% VidLoc~\cite{Clark:VidLoc:CVPR2017} required to training and testing in same environment, although it could resume absolute scale pose. 
 

% \end{itemize}
%\end{flushleft}

\noindent\textbf{Beyond supervised learning.} Most of deep learning based methods for visual localization are fully supervised. As noted, ground truth data collection is non-trivial. Therefore, a few alternative learning strategies have been investigated as well. Unsupervised learning, for example, avoids labeled data collection. The recent DeepMapping~\cite{Ding:DeepMapping:CVPR19} introduces an unsupervised framework for multiple point clouds registration and mapping, where the supervision signals are derived from the free-space consistency among point clouds. The trained model is able to perform coarse re-localization for unseen point clouds that are in close vicinity to the registered point clouds. The main drawback of this method is that it is only applicable to point cloud modality. Besides, weakly supervised learning provides weak supervision that can be easily obtained, such as inaccurate, incomplete, or inexact ground truth data~\cite{Zhou:IntroWeakSup:NSR18}. For example, method in~\cite{Stewart:PhyConstraintSupervision:AAAI17} introduces a physical-based constraint for detecting and tracking free-falling objects in the video where the heights of the detected objects should be a parabola.


%\textbf{Related work conclusion} 
% \begin{itemize}
    %\item Majority of pioneer’s methods on place recognition and visual odometry required supervised learning. They relocalize position and estimate observation pose by feature extraction as advantage of CNN and time series regression on LSTM. LS-VO [……] The performance of APR strongly relies on the quantity and the quality of training data available. High-quality annotation of the camera pose for each image, however, is not a trivial task and poses a challenge for these supervised learning approach.
    
    %\item unsupervised/ self-supervised
    
    % \item The recent DeepMapping~\cite{Ding:DeepMapping:CVPR19} introduces an unsupervised framework for multiple point clouds registration and mapping. The trained model is able to perform coarse re-localization for unseen point clouds. Pros: does not required ground truth sensor poses for training. The entire framework is unsupervised. Cons: unseen point clouds must be in close vicinity to the registered point clouds and have a similar orientation. occupancy consistency loss only applicable to point cloud



% \end{itemize}
%\end{flushleft}

